Scalable Multi-Output Label Prediction: From Classifier Chains to Classifier Trellises

Multi-output inference tasks, such as multi-label classification, have become increasingly important in recent years. A popular method for multi-label classification is classifier chains, in which the predictions of individual classifiers are cascaded along a chain, thus taking into account inter-label dependencies and improving the overall performance. Several varieties of classifier chain methods have been introduced, and many of them perform very competitively across a wide range of benchmark datasets. However, scalability limitations become apparent on larger datasets when modeling a fully-cascaded chain. In particular, the methods' strategies for discovering and modeling a good chain structure constitutes a mayor computational bottleneck. In this paper, we present the classifier trellis (CT) method for scalable multi-label classification. We compare CT with several recently proposed classifier chain methods to show that it occupies an important niche: it is highly competitive on standard multi-label problems, yet it can also scale up to thousands or even tens of thousands of labels.

==> tableRunningTimePR3.tex <==
\begin{tabular}{lrrrrrrr}
\hline
Dataset   & \alg{IC}&\alg{ECC}&\alg{MCC}&\alg{EBCC}&\alg{CT}&\alg{ECT}&\alg{CDT} \\
\hline
Music                &      1 (3) &      5 (7) &      4 (6) &      2 (5) &      1 (1) &      2 (4) &      1 (2)  \\ 
Scene                &      3 (1) &     10 (5) &     28 (7) &      7 (3) &      4 (2) &     12 (6) &     10 (4)  \\ 
Yeast                &     12 (2) &     56 (6) &     83 (7) &     46 (5) &      6 (1) &     28 (4) &     13 (3)  \\ 
Medical              &      8 (2) &     47 (5) &     77 (6) &     43 (4) &      5 (1) &     40 (3) &    145 (7)  \\ 
Enron                &     54 (2) &    319 (5) &    742 (7) &    113 (3) &     28 (1) &    144 (4) &    347 (6)  \\ 
TMC07                &  11409 (2) &  48069 (6) &  73436 (7) &  34601 (4) &  10854 (1) &  45062 (5) &  14081 (3)  \\ 
MediaMill            &     57 (1) &    558 (4) &   1152 (5) &    381 (3) &     78 (2) &   1191 (6) &   5524 (7)  \\ 
Delicious            &    635 (1) &    DNF     &  18955 (4) &    DNF     &    735 (2) &  10323 (3) &  32584 (5)  \\ 
Local400       &      3 (1) &     32 (5) &     61 (6) &     18 (3) &      3 (2) &     26 (4) &    430 (7)  \\ 
Local10k         &      7 (1) &    DNF     &    DNF     &     31 (3) &      7 (2) &     53 (4) &   4231 (5)  \\ 
\hline
avg rank  &  1.60      &  5.38      &  6.11      &  3.67      &  1.50      &  4.30      &  4.90      \\
\hline
% mean(avg. rank)=3.92182539683
% CD=2.60168517183
% 3.92182539683 > 2.60168517183 ?
% -> Reject the null hypothesis because the average rank difference > CD
\end{tabular}

